Covert Multi-Access Communication with a Non-Covert User

In this paper, we characterize the fundamental limits of a communication system with three users (i.e., three transmitters) and a single receiver where communication from two covert users must remain undetectable to an external warden. Our results show a tradeoff between the highest rates that are simultaneously achievable for the three users. They further show that the presence of a non-covert user in the system can enhance the capacities of the covert users under stringent secret-key constraints. To derive our fundamental limits, we provide an information-theoretic converse proof and present a coding scheme that achieves the performance of our converse result. Our coding scheme is based on multiplexing different code phases, which seems to be essential to exhaust the entire tradeoff region between the rates at the covert and the two non-covert users. This property is reminiscent of the setup with multiple non-covert users, where multiplexing is also required to exhaust the entire rate-region.

==> contents/abstract.tex <==
\begin{abstract}
We establish the fundamental limits of a three-user single-receiver system where communication from User 1 and User 2 (but not from User 3) must remain undetectable to an external warden. 
Our findings reveal a tradeoff between the highest rates that are simultaneously achievable for the three users. 
Interestingly, the presence of the non-covert user can enhance the capacities of the covert Users 1 and 2, especially under stringent secret-key budgets. 
% In addition to that, we show through simulation as well that a coded time-sharing strategy is fundamentally required to increase the covert capacity, which distinguishes this setup from the more classical setups with either only covert users or only non-covert users. 
In addition, our findings underscore the essential requirement of employing a {\color{red}coded time-sharing strategy} to increase the covert capacity, setting this setup apart from more conventional configurations featuring either exclusively covert or non-covert users.
\end{abstract}

\begin{IEEEkeywords}
Physical Layer Security, Covert Communication, Undetectable Communication, IoT
\end{IEEEkeywords}

==> contents/achievability.tex <==
\section{Proof Of Theorem~\ref{main_theorem}}\label{sec:coding}
% As stated in Section~\ref{sec:coding_overview}, the achievability analysis relies on the standard random coding argument. 
% The main difference here being that the probability of sending the $1$ symbol at the covert users vanishes in the blocklength $n$ (approximately in the order of $1/\sqrt{n}$).
Our main results are an achievability result for finite blocklengths and a converse that asymptotically matches this achievability analysis.
For brevity of the description, we omit the details of the proofs that are same to that of \cite{ours_first}. Instead, we provide discussions and intuitions to help understanding.

For any pair $(x_3, t) \in \mathcal{X}_3 \times \mathcal{T}$ and non-negative real values $\rho_{1, t}, \rho_{2, t} \in \mathbb{R}_0^+$, where $\mathcal{T}$ is the time set, we define:
\begin{IEEEeqnarray}{rCl}
    % \!\!\!\!\!\!\!\!\chi_n^2(\bm{\rho}_t, x_3) &\triangleq& \sum_{z \in \mathcal{Z}} \frac{1}{\Gamma_{00x_3}(z)} \Big[\mu_{1,t} \Gamma_{10x_3}(z) + \mu_{2,t} \Gamma_{01x_3}(z) \nonumber \\ 
    % &-& \Gamma_{00x_3}(z)  + \mathcal{O}\left(\alpha_n^2 \right)\Big]^2
    \!\!\!\!\!\!\chi_n^2(\bm{\rho}_t, &x_3&) \triangleq \sum_{z \in \mathcal{Z}} \frac{1}{\Gamma_{00x_3}(z)} \Big[\frac{\rho_{1,t}}{\rho_{1,t} + \rho_{2,t}} \Gamma_{10x_3}(z) \nonumber \\ 
    &+& \frac{\rho_{2,t}}{\rho_{1,t} + \rho_{2,t}} \Gamma_{01x_3}(z) - \Gamma_{00x_3}(z)  + \mathcal{O}\left(\alpha_n^2 \right)\Big]^2. \label{eq:def_xi_n_distance}
\end{IEEEeqnarray}
Notice that $\chi^2(\bm{\rho}_t, x_3) = \lim_{n\to \infty} \chi_n^2(\bm{\rho}_t, x_3)$.
% % As for the decoding, the non-covert message is decoded first, then the covert messages are decoded by a Treating Interference as Noise (TIN) scheme as is the case in \cite{tin_paper}, where it has been shown to be optimal for a $K$-user MAC.

% \underline{\textit{Preparations:}}\\
% %Let $\mathcal{T}$, $P_T$, $\{\epsilon_t\}$, and $P_{X_{1,n}|T}$ and $P_{X_2}$ be given as in the theorem. 
% Let $\omega_n$ be a sequence satisfying \eqref{eq:lim_omega_n_def}.
% For each $t \in \mathcal{T}$, define  the conditional pmfs
% \begin{IEEEeqnarray}{rCl}
% P_{X_{1,n} \mid T}(1 \mid t)=1-P_{X_{1,n} \mid t}(0 \mid t) \triangleq \rho_{1,t} \alpha_{n}\\
% P_{X_{2,n} \mid T}(1 \mid t)=1-P_{X_{2,n} \mid t}(0 \mid t) \triangleq \rho_{2,t} \alpha_{n} 
% \end{IEEEeqnarray}
% and let  $\mu_{n}\triangleq n^{-1/3}$ and   the type  $\pi$   over $\mathcal{T}^n$ satisfy
% \begin{IEEEeqnarray}{rCl}
%     \left | \pi(t) - P_T(t) \right | \leq \mu_n \quad \forall t \in \mathcal{T},
% \end{IEEEeqnarray}
% as well as $\pi(t)=0$ whenever $P_T(t)=0$. Fix a large blocklength $n$ and let $t^n=(t_1,\ldots, t_n)$ be of type $\pi$. 

% Define the joint pmf
% \begin{equation}\label{eq:Pn}
% P_{TX_1X_2X_3Y}^{(n)}\triangleq P_{TX_3}P_{X_{1,n} \mid T}P_{X_{2,n} \mid T}W_{Y \mid X_1X_2X_3}.
% \end{equation}

% Let $P_{TX_3Y}$ denote the $(T,X_3,Y)$-marginal of the pmf $P_{TX_1X_2X_3Y}^{(n)}$ and notice that the following asymptotic quantity exists  because  $\alpha_n \to 0$:
% \begin{IEEEeqnarray}{rCl}
% \!\!\!\!\!\!\!\!\!P_{TX_3Y}^*(t,x_3,y) &\triangleq& \lim_{n\to\infty} P_{TX_3Y}^{(n)}(t,x_3,y) \\
% &=& P_{ TX_3}(t,x_3)W_{Y|X_1X_2X_3}(y|0,0,x_3).
% \end{IEEEeqnarray}
% \textit{Codebook generation:}
% \begin{itemize}
%     \item For user 1,  generate a codebook
%     \begin{equation}\mathcal{C}_{1} =  \left \{  x_{1}^{n}(1,1), \ldots, x_{1}^{n}\big(2^{M_{1}},2^{K_1}\big) \right \}  \end{equation}
%     by drawing the $i$-th entry of codeword $x_1^n(w_1,s_1)$ according to the pmf $P_{X_{1,n} \mid T}(\cdot|t_i)$ independent of all other entries.

%     \item For user 2,  generate a codebook
%     \begin{equation}\mathcal{C}_{2} =  \left \{  x_{2}^{n}(1,1), \ldots, x_{1}^{n}\big(2^{M_{2}},2^{K_2}\big) \right \}  \end{equation}
%     by drawing the $i$-th entry of codeword $x_2^n(w_2,s_2)$ according to the pmf $P_{X_{2,n} \mid T}(\cdot|t_i)$ independent of all other entries.

%     \item For user 3,  generate a codebook
%     \begin{equation}\mathcal{C}_3 =  \left \{ \left. x_{3}^{n}(1) , \ldots, x_{3}^{n}\big(2^{nr_{3}}\big) \right \} \right. \end{equation}
%         by drawing the codewords independent of each other and each entry i.i.d.  according to the pmf $P_{X_{3} \mid T}(\cdot|t_i)$. 
% \end{itemize}
% Notice that while both pmfs $P_{X_{1,n} \mid T}$ and $P_{X_{2,n} \mid T}$ used to construct $\mathcal{C}_1$ and $\mathcal{C}_2$ depends on the blocklength $n$, the pmf $P_{X_3|T}$ used to construct $\mathcal{C}_3$ is independent of $n$ as user 3 does not have to be covert.

% \underline{\textit{Encoding and Decoding:}}\\
% If $\mathcal{H}=1$ User 1 and User 2 send the codewords $x_1^n(W_1,S_1)$ and $x_2^n(W_2,S_2)$ respectively, and if $\mathcal{H}=0$ they sends $x_1^n=0^n$ and $x_2^n=0^n$ respectively. User 3 however sends the codeword $x_3^n(W_3)$ whatever the hypothesis $\mathcal{H}$ as it's not aware of it.

% The legitimate receiver, who observes $Y^n=y^n$ and knows the secret keys $(S_1,S_2)$ and the hypothesis $\mathcal{H}$, performs successive decoding starting with message  $W_3$ followed by the messages $W_1$ and $W_2$. 

% \textit{\underline{When $\mathcal{H}=0$}}: the legitimate receiver looks for a unique index $w_{3}$ satisfying 
% \begin{equation}\label{eq:decoding2}
% (t^n,x_3^{n}(w_3), y^{n}) \in \mathcal{T}_{\mu_n}^{n}(P_{TX_3Y }).
% \end{equation}
% If such a unique index  $w_3$ exists, the receiver sets $\widehat{W}_3=w_3$. Otherwise it declares an error and stops.

% % \textit{When $\mathcal{H}=0$}: both User 1 and User 2 sends the sequences $x_1^n(W_1,S)=0^n$ and $x_2^n(W_2,S)=0^n$. Since the legitimate receiver is aware of the hypothesis $\mathcal{H}$, he does not perform anything in this scenario.\\

% \textit{\underline{When $\mathcal{H}=1$}}: After decoding the message $W_3$, the receiver tries to decodes also the messages of the covert users (User 1 and User 2) following a TIN scheme. For all $k \in \{1,2\}$ we define the set $\mathcal{A}_{\eta_k}^{n}$ in \eqref{eq:set_a_gamma_n_def_achievability} on top of next page
% \begin{figure*}
%     \begin{IEEEeqnarray}{rCl}
%         \label{eq:set_a_gamma_n_def_achievability}
%         \mathcal{A}_{\eta_k}^{n} \triangleq \left \{  (x_{1}^{n}, x_{2}^{n} ,x_3^{n}, y^{n}) \in  \mathcal{X}_1^{n} \times \mathcal{X}_2^{n} \times \mathcal{X}_3^{n} \times \mathcal{Y}^{n} : \log \left( \frac{W_{Y|X_1X_2X_3}^{\otimes n}(y^{n} | x_{1}^{n}, x_{2}^{n}, x_3^n) }{W_{Y|X_1X_2X_3}^{\otimes n}(y^{n} |0^n, 0^n, x_3^n) }  \right) \geq \eta_k \right \}.
%     \end{IEEEeqnarray}
%     \hrule 
% \end{figure*}
%  where $\eta_k$ are positive constants that will be defined later.  
% To decode the message $W_1$, the legitimate receiver first sets $x_2^n(W_2,S_2) = 0^n$ and looks for a unique index $w_1$ satisfying 
% \begin{equation}\label{eq:decoding1}
% (x_{1}^{n}(w_1, S_1), 0^n,x_3^{n}(\widehat{W}_3), y^{n})\in \mathcal{A}_{\eta_1}^{n},
% \end{equation} 
% If such a unique index  $w_1$ exists, the receiver sets $\widehat{W}_1=w_1$. Otherwise it declares an error and stops. The receiver next looks for a unique index $w_2$ satisfying 
% \begin{equation}
% (0^n,x_{2}^{n}(w_2, S_2),x_3^{n}(\widehat{W}_3), y^{n}) \in \mathcal{A}_{\eta_2}^{n}).
% \end{equation}
% If such a unique index  $w_2$ exists, the receiver sets $\widehat{W}_2=w_2$. Otherwise it declares an error and stops.
\subsubsection{Auxiliary Lemmas} \label{sec:auxiliary_lemmas}
Before we present our proof, we present some lemmas that are essential for the achievability analysis.
\begin{lemma}\label{lem:aux}
For each blocklength $n$ let $\omega_n$ be a sequence satisfying \eqref{eq:lim_omega_n_def}. For each $t \in \mathcal{T}$, let also $\rho_{1,t}, \rho_{2,t}$ be positive constants in $\mathbb{R}_0^+$. There exists a sequence of encoding and decoding functions $\{(\varphi_1^{(n)}, \varphi_2^{(n)}, \phi_1^{(n)}, g_1^{(n)}, g_2^{(n)})\}_n$ satisfying the conditions in Theorem~\ref{main_theorem} and moreover
\begin{IEEEeqnarray}{rCl}
\frac{1}{M_3} \sum_{w_3=1}^{M_3} \delta_{n,w_3} & = & ( 1+ o(1)) \frac{\omega_n^2 }{2} \mathbb{E}_{P_{TX_3}} \Big[ (\rho_{1,T} + \rho_{2,T})^2  \nonumber \\
&\cdot& \chi_n^2(\bm{\rho}_T,X_3) \Big ] \IEEEeqnarraynumspace \label{eq:aux}
\end{IEEEeqnarray}
for a function $o(1)$ that tends to 0 as $n\to \infty$.
\end{lemma}
\begin{IEEEproof}
% By inspecting the proof of Theorem~\ref{main_theorem}. The proof is similar to~\cite[Lemma 1]{ours_first} and is omitted.
By inspecting the proof of Theorem~\ref{main_theorem}. The proof is similar to~\cite[Lemma 1]{ours_first} and is omitted in this paper.
\end{IEEEproof}
% \highlight{
% \begin{lemma}
%     \label{lem:convexity}
%     The set of four-dimensional vectors $(r_1, r_2, r_3, k)$ satisfying inequalities $\eqref{eq:asymp1}-\eqref{eq:asympkey}$ for some choice of pmfs $P_{TX_3}$ and values $\rho_{k,t} \in \mathbb{R}^{+}_0$ for all $(k,t) \in \{1,2\} \times \mathcal{T}$ is a convex set.
% \end{lemma}
% \begin{IEEEproof}
% The proof is an extension of~\cite[Lemma 2]{ours_first} and is omitted. 
% \end{IEEEproof}
% }
The following lemma is an immediate consequence of previous works \cite[Lemma~1]{bloch_k_users_mac}.
\begin{lemma}
\label{lemma_1_asymptotics}
For each blocklength $n$, consider two conditional pmfs $P_{X_{1,n} \mid T}$ and $P_{X_{2,n} \mid T}$ over the binary alphabets $\mathcal{X}_1$ and $\mathcal{X}_2$ respectively, such that for any $t \in \mathcal{T} $ and $\rho_{1,t}, \rho_{2,t} \in \mathbb{R}_{0}^+$, the two pmfs satisfies $P_{X_{1,n} \mid T}(1 \mid t) \triangleq \rho_{1,t} \alpha_{n} \to 0$ and $P_{X_{2,n} \mid T}(1 \mid t) \triangleq \rho_{2,t} \alpha_{n} \to 0$ in the limit of large blocklength $n$.
Define  for each $x_3 \in \mathcal{X}_3$ and $z \in \mathcal{Z}$:
\begin{IEEEeqnarray}{rCl}
    W_{Z \mid X3}^{(t)} (z \mid x_3) \triangleq \!\!\sum_{(x_1,x_2) \in \mathcal{X}_1 \times \mathcal{X}_2} \!\!\!\!\!\!&&P_{X_{1,n} \mid T}(x_1 \mid t) P_{X_{2,n} \mid T}(x_2 \mid t) \nonumber \\
    && \cdot \Gamma_{x_1x_2x_3}(z).
\end{IEEEeqnarray}
Then, for all sufficiently large values of $n$: 
\begin{align}
    \label{eq:lemma1_denominator_bound_for_achievability}
    &(1-\epsilon_n) \cdot \frac{\left[ \left(  \rho_{1,t} + \rho_{2,t}\right) \alpha_n \right]^2}{2} \chi_n^2(\bm{\rho}_t, x_3) \nonumber \\
    &\leq \mathbb{D}( W_{Z \mid X3}^{(t)} (\cdot \mid x_3) \|\Gamma_{00x_3}) \nonumber \\
    &\leq   (1+\epsilon_n) \cdot \frac{\left[ \left(  \rho_{1,t} + \rho_{2,t}\right) \alpha_n \right]^2}{2} \chi_n^2(\bm{\rho}_t, x_3). 
\end{align}
where we define a sequence $\{ \epsilon_n \}_{n \geq 1}$ of positive elements, such that
\begin{equation}
    \lim_{n \to \infty} \epsilon_n = 0,
\end{equation}
\end{lemma}
\begin{IEEEproof}
This lemma is essential for the achievability analysis and the proof is fundamentally an extension of the proof of~\cite[Lemma 1]{bloch_k_users_mac}.
\end{IEEEproof}
Notice that the tuple $\bm{\rho_t}$ represents how we allocate the number of $1$ symbols for each of the covert users at each time instance $t \in \mathcal{T}$. 
Intuitively, Lemma~\ref{lemma_1_asymptotics} suggests that for each non-covert symbol $x_3 \in \mathcal{X}_3$, the chi-square distance $\chi_n^2(\bm{\rho}_t, x_3)$ controls covertness and is common to the two covert users' rates as communication of each of them jointly affects the covertness constraint.
More specifically, Lemma~\ref{lemma_1_asymptotics} provides an insightful characterization of how the number of $1$ symbols associated with each covert user influences the relative entropy of interest through the power allocation vector $\bm{\rho_t}$ at each time instance and the chi-squared distance between the mixture output distribution and the output distribution when the non-covert user is the only one communicating. 
In fact, and as we shall see in Section~\ref{sec:channel_resolvability_analysis}, it only matters to make the divergence term in \eqref{eq:lemma1_denominator_bound_for_achievability} small to allow covert communication for user 1 and user 2.
\subsubsection{Error Probability Analysis} \label{sec:error_proba_analysis}
The proposed coding scheme allows for an elegant extension of our recent results~\cite{ours_first}. 
One can show that for any $k \in \{1,2\}$ and for any $\mu_k > 0$ and $\xi_k > 0$, such that $\mu_k < \xi_k$ the choices
% \begin{IEEEeqnarray}{rCl}
%     \eta_k &\triangleq& (1-\mu_k) \omega_n \sqrt{n}  \mathbb{E}_{P_{TX_3}} \left[ \rho_{k,T} D_{Y}^{(k)}(X_3) \right], \label{eq:value_eta_k_achievability} \\
%     \log(M_k) &\triangleq& (1-\xi_k) \omega_n \sqrt{n}  \mathbb{E}_{P_{TX_3}} \left[ \rho_{k,T} D_{Y}^{(k)}(X_3) \right],  \label{eq:choice_for_alphabet_size}
% \end{IEEEeqnarray}
% and
% \begin{IEEEeqnarray}{rCl}
%     \log(M_3) &\triangleq& (1-\xi_3) n \mathbb{I}(X_3;Y \mid X_1=0,X_2=0,T),  \label{eq:choice_for_alphabet_size_non_covert}
% \end{IEEEeqnarray}
\begin{IEEEeqnarray}{rCl}
    \eta_k &\triangleq& (1-\mu_k) \omega_n \sqrt{n}  \mathbb{E}_{P_{TX_3}} \left[ \rho_{k,T} D_{Y}^{(k)}(X_3) \right], \label{eq:value_eta_k_achievability} \\
    \log(M_k) &\triangleq& (1-\xi_k) \omega_n \sqrt{n}  \mathbb{E}_{P_{TX_3}} \left[ \rho_{k,T} D_{Y}^{(k)}(X_3) \right],  \label{eq:choice_for_alphabet_size} \\
    \log(M_3) &\triangleq& (1-\xi_3) n \mathbb{I}(X_3;Y \mid X_1=0,X_2=0,T),  \label{eq:choice_for_alphabet_size_non_covert}
\end{IEEEeqnarray}
are sufficient to make the probability of errors in \eqref{eq:prob2} and \eqref{eq:prob1} sufficiently small so as to allow for a reliable covert communication for user 1 and user 2, and a reliable communication for user 3.
The proof follows by the lines of~\cite{ours_first}.
Combining \eqref{eq:value_eta_k_achievability}-\eqref{eq:choice_for_alphabet_size_non_covert} and Lemma~\ref{lem:aux} yields \eqref{eq:asymp1}-\eqref{eq:asymp3}.
\subsubsection{Channel Resolvability Analysis} \label{sec:channel_resolvability_analysis}
As is common knowledge, coding introduces structure. While one can make the probability of sending the $1$ symbol at the covert users very small, an efficient adversary can look at the structure of the code to infer whether communication is happening or not. To make the output distribution at the warden close to an i.i.d. process, we resort to channel resolvability techniques (also know as approximation of output statistics) as introduced in~\cite{bloch_first}. In particular, these techniques will allow us to find the minimum secret-key length that is required so as to emulate the i.i.d. process and thereby destroying the structure for anyone not aware of the secret-key.

Start by noticing the following:
\begin{IEEEeqnarray}{rCl} 
    \label{eq:resolvability_original}
    &&\!\!\!\!\!\!\!\!\!\!\!\Bigg | \mathbb{D}\left( \widehat{Q}_{\mathcal{C}, w_3}^n \Big\| W^{\otimes n}_{Z|X_1X_2X_3} ( \cdot | 0^n, 0^n, x_3^n(w_3))\right) \nonumber \\
    &-&  \mathbb{D}\left( \Tilde{W}_{Z^n \mid X_3^n} \Big\| W^{\otimes n}_{Z|X_1X_2X_3} ( \cdot | 0^n, 0^n, x_3^n(w_3))\right) \Bigg | \nonumber \\
    &\leq& \sqrt{\mathbb{D}\left( \widehat{Q}_{\mathcal{C}, w_3}^n \Big\| \Tilde{W}_{Z^n \mid X_3^n}\right)} \left( 1 + \frac{n}{\sqrt{2}} \log\left( \frac{1}{\eta_0} \right)\right ). \label{eq:abs_diff}
\end{IEEEeqnarray}
where $\eta_0$ is defined as the minimum probability in the support of $\Gamma_{00x3}$ and
\begin{IEEEeqnarray}{rCl}    
\label{eqn:def_Q_tilde_n}
   \Tilde{W}_{Z^n \mid X_3^n}(z^n \mid x_3^n) \triangleq \prod_{i=1}^n W_{Z \mid X_3}^{(t_i)}(z \mid x_3).
\end{IEEEeqnarray}
Notice also that by construction, $\Tilde{W}_{Z^n \mid X_3^n} \underset{\infty}{\rightarrow} W^{\otimes n}_{Z|X_1X_2} ( \cdot | 0^n, 0^n, x_3^n(w_3))$.
Thus, in view of~\eqref{eq:abs_diff}, 
covertness is established by proving that the expected divergence
\begin{equation}\label{eq:D1}
   \mathbb{E}_{\mathcal{C}}\left[\mathbb{D}\left( \widehat{Q}_{\mathcal{C}, w_3}^n \Big\| \Tilde{W}_{Z^n \mid X_3^n}(z^n \mid X_3^n)\right) \right]
\end{equation}  
vanishes  in the  blocklength $n$.
One can show that if
\begin{IEEEeqnarray}{rCl}
 \log(K_1K_2) &\triangleq& (1-\xi_4) \omega_{n}\sqrt{n} \mathbb{E}_{P_{TX_3}}  \Big[ \sum_{k=1}^{2}\rho_{k,T} D_{Z-Y}^{(k)}(X_3) \Big], \nonumber \\ 
\end{IEEEeqnarray}
the quantity in~\eqref{eq:D1} vanishes exponentially fast in $n$. 
The proof follows by the lines of~\cite{ours_first} and is omitted for brevity of presentation.

\subsubsection{Converse Proof} \label{sec:converse_proof}
% The converse proof presented in~\cite{ours_first} can be extended to this setup.
The converse proof that we initially introduced in~\cite{ours_first} can be readily extended to accommodate the specific setup under consideration. 
This extension leverages the fundamental principles and insights established in the referenced work to aptly address the nuances and complexities inherent to this setup.

==> contents/coding_scheme_main_result_and_simulations.tex <==
\section{Coding Scheme, Main Result, and Numerical Simulations}
\label{sec:coding_and_simulation}

\subsection{Coding Scheme}
\label{sec:coding_overview}
Our coding scheme operates in $\tau$\footnote{We will see that $\tau=5$ suffices.}  different phases $t=1, 2, \ldots, \tau$. Multiple phases are required by the multi-objective nature of our communication that not only wishes to minimize various error probabilities but also the divergence between the output distribution observed at the warden under the two hypotheses (so as to reduce its detection capability). While certain phases will provide small probabilities of error, other phases will induce small divergences. The combined scheme over all phases  then induces an optimal overall-tradeoff between small probabilities of error and small divergences.

Specifically, we split the entire blocklength $n$ into $\tau$ transmission phase $t=1,2,\ldots, \tau$ of lengths $n_1,n_2, \ldots, n_{\tau}$. 

\textit{\underline{Code construction:}} 
We pick two
non-detectable multiple-access codes  \cite{bloch_k_users_mac} $\mathcal{C}_{1,t}$ and $\mathcal{C}_{2,t}$ for the transmission of the two covert messages $W_1$ and $W_2$. By construction \cite{bloch_k_users_mac, tin_paper, ours_first}, codebooks  $\mathcal{C}_{1,t}$ and $\mathcal{C}_{2,t}$ contain codewords $\big\{x_{1,t}^{n_t}(W_1, S_1)\big\}$ and $\big\{x_{2,t}^{n_t}(W_2, S_2)\big\}$ that depend on the respective messages as well as the corresponding secret keys $S_1$ and $S_2$.

An important parameter of the covert-communication codes $\mathcal{C}_{1,t}$ and $\mathcal{C}_{2,t}$ are the average number of $1$-symbols in the codewords. Covert codewords of length $n$  typically contain $\rho \cdot \omega_n \sqrt{n}$ occurrencies of the  $1$-symbols for a fixed prefactor $\rho$ independent of $n$ and a sequence $\omega_n$ that decays to 0 but slower than $n^{-1/2}$. We denote the prefactors of the chosen covert codes by $\mathcal{C}_{k,t}$ by $\rho_{k,t}$.

Standard (non-covert) single-user codes $\mathcal{C}_{3,t}$, for $t=1,\ldots, \tau$ are used  for the transmission of the non-covert message $W_3$ in the different phases. The codewords $x_{3,t}^{n_t}(W_3)$ depend only on message $W_3$. A key parameter of these codes is again the frequency  of the various symbols in the codewords, which we denote by $P_{X_3|t}$ for codebook $\mathcal{C}_{3,t}$. It is typically fixed and independent of the blocklength. 


\textit{\underline{Encoding:}} User $3$ concatenates codewords 
\begin{equation}
x_{3,1}^{n_1}(W_3) , \; x_{3,2}^{n_2}(W_3),\;  \ldots, \; x_{3,\tau}^{n_\tau}(W_3)
\end{equation}
and sends the resulting string over the channel.

Under $\mathcal{H}=0$ Users 1 and 2 send the all-zero sequences $x_1^n=0^n$ and $x_2^n=0^n$. Under $\mathcal{H}=1$ Users 1 and 2 concatenate the codewords from the different codebooks
\begin{eqnarray}
x_{k,1}^{n_1}(W_k,S_k) , \; x_{k,2}^{n_2}(W_k,S_k),\;  \ldots, \; x_{k,\tau}^{n_\tau}(W_k,S_k),  \nonumber \\
\hspace{5cm} \qquad k=1,2,
\end{eqnarray}
and send the resulting strings over the channel. 

%Since the warden should not be able to detect whether  $x_1^n$ and $x_2^n$ are the all-zero sequences or correspond to a concatenation of codewords, by construction they cannot contain too many $1$-symbols. In fact, it can be shown \cite{ligong} that the number of  $1$-symbols over the entire blocklength $n$ should only be in the order of $\sqrt{n}$. 
% see Figure~\ref{fig:coding_scheme}. 
%In each phase, for the non-covert user, we generate the codewords using a conventional code \cite{cover}, whereas for the covert users, we leverage the well-established covert code in the literature i.e. a code with vanishing probability of sending the $1$-symbol in the blocklength $n$ (approximately in the order of $1/\sqrt{n}$). 
%More formally, let $\omega_n$ be a sequence satisfying

%and define
%\begin{IEEEeqnarray}{rCl}
%    \alpha_n &\triangleq& \frac{\omega_n}{\sqrt{n}}.
%\end{IEEEeqnarray}
%For each covert user $u_c\in \{1,2\} $ and a time instance $t \in \{1,\ldots, 5\}$ we have
%\begin{equation}
%    P_{X_{u_c,n}}(X_{u_c} = 1 \mid T=t) = \rho_{u_c,t} \alpha_n.
%\end{equation}
%As our forthcoming numerical simulations will elucidate, coded time-sharing significantly enhances the covert capacity and we shall also give some intuitions behind why it is the case in Section~\ref{sec:simulations}.

%\begin{figure}[!h]
%    \centering
%    \includegraphics[scale=0.6]{figures/timesharing_3_users_T=5.pdf}
%    \caption{Structure of our coding scheme.}
%    \label{fig:coding_scheme}
%\end{figure}
\textit{\underline{Decoding:}}
The legitimate receiver employs a successive decoding procedure starting with the non-covert message of User 3 and followed by the two covert messages, which can be decoded in parallel. Details are as follows: 
\begin{enumerate}
\item The receiver first decodes message $W_3$ assuming that Users 1 and 2 send the all-zero sequences (irrespective of whether $\mathcal{H}=0$ or $\mathcal{H}=1$). Even under $\mathcal{H}=1$ this assumption will not distort the problem too much because the number of $1$-symbols is small (in the order of $\sqrt{n}$) anyways.
\item Having decoded  the non-covert message $W_3$, the receiver proceeds with decoding either message $W_1$ or message  $W_2$. Assume it starts by decoding $W_1$ using a standard decoding rule for the covert-codes $\mathcal{C}_{1,t}$. For this decoding step the receiver can again assume that $x_2^n=0^n$. 
\item The receiver proceeds to decode the second covert message $W_2$ using a standard decoding rule for the covert-codes $\{\mathcal{C}_{2,t}\}$ and assuming that User 1 sent the all-zero sequence  $x_1^n=0^n$. 
\end{enumerate}

Steps 2) and 3) can be inverted or even be ran in parallel. It is however important that Step 1) is executed first. 


\subsection{Main Results}
For ease of notation, define\begin{IEEEeqnarray}{rCl}
W_{x_1x_2x_3}(y) &\triangleq& W_{Y|X_1X_2X_3}(y \mid x_1, x_2, x_3),\\
\Gamma_{x_1x_2x_3}(z) &\triangleq& \Gamma_{Z|X_1X_2X_3}(z \mid x_1, x_2, x_3),
\end{IEEEeqnarray}
%for any $x_1 \in \mathcal{X}_1, x_2 \in \mathcal{X}_2, x_3 \in \mathcal{X}_3, y \in \mathcal{Y},$ and $z \in \mathcal{Z}$.
%Moreover, for any $x_3 \in \mathcal{X}_3$, we define:
and 
\begin{IEEEeqnarray}{rCl}
D_{Y}^{(1)}(x_3)& \triangleq & \mathbb{D} \left(W_{10x_3} \mid \mid W_{00x_3}  \right), \\
D_{Y}^{(2)}(x_3)& \triangleq & \mathbb{D} \left(W_{01x_3} \mid \mid W_{00x_3}  \right), \\
D_{Z}^{(1)}(x_3)& \triangleq & \mathbb{D} \left(\Gamma_{10x_3} \mid \mid \Gamma_{00x_3}  \right), \\
D_{Z}^{(2)}(x_3)& \triangleq & \mathbb{D} \left(\Gamma_{01x_3} \mid \mid \Gamma_{00x_3}  \right), \\
D_{Z-Y}^{(k)}(x_3) & \triangleq &  D_{Z}^{(k)}(x_3) - D_{Y}^{(k)}(x_3), \quad \forall k \in \{1,2\} ,\IEEEeqnarraynumspace
\end{IEEEeqnarray}
where $\mathbb{D}(P \| Q)$ denotes the Kullback-Leibler divergence between $P$ and $Q$.

Also, we use the abbreviation $\bm{\rho}_t \triangleq (\rho_{1,t}, \rho_{2,t})$ 
and define for each $x_3 \in \mathcal{X}_3$: 
\begin{IEEEeqnarray}{rCl}
\chi^2(\bm{\rho}_t, x_3) &\triangleq& \sum_{z \in \mathcal{Z}} \left[\frac{\rho_{1,t}}{\rho_{1,t} + \rho_{2,t}}\frac{ \Gamma_{10x_3}(z)}{\Gamma_{00x_3}(z)} \nonumber \right.\\ 
    &&\left.\hspace{.8cm}+ \frac{\rho_{2,t}}{\rho_{1,t}+ \rho_{2,t}} \frac{\Gamma_{01x_3}(z)}{\Gamma_{00x_3}(z) } -1\right]^2. \label{eq:def_xi_distance}\IEEEeqnarraynumspace
\end{IEEEeqnarray}

%Essentially, $\chi^2(\bm{\rho}_t, x_3)$ is a chi-squared distance between two output distributions at the warden. 

%Our main results are:
%We characterized the performances of the optimal code for this communication setup. We first present a finite blocklength result in Theorem~\ref{main_theorem} then an asymptotic result in Theorem~\ref{th:asymp_result}.
\medskip
%Let $\mathcal{T} \triangleq \{1, \ldots, 5\}$.
\begin{theorem}
\label{main_theorem}
For any $\epsilon>0$ and sufficiently large blocklengths $n$ there is a suitable choice of the codes $\mathcal{C}_{1,t}, \mathcal{C}_{2,t}, \mathcal{C}_{3,t}$, for $t=1, \ldots, \tau$, for which the coding scheme described in the previous subsection achieves probability of error $P_e\leq \epsilon$ 
and 
average warden divergence
\begin{equation}
\frac{1}{M_3} \sum_{w_3=1}^{M_3} \delta_{n, w_3} \leq  (1+\xi_1) \frac{\omega_n^2}{2} \mathbb{E}\left[ (\rho_{1,T}+\rho_{2,T})^2 \cdot \chi^2(\bm{\rho}_T, X_3)\right],
\end{equation}
whenever the following conditions hold: 
%Let the  pair of  random variables  $(T,X_3)$ over $\mathcal{T} \times \mathcal{X}_3$ be distributed according to  a pmf $P_{TX_3}$. 
%Let also $\{\omega_{n}\}_{n=1}^\infty$ be a sequence satisfying 
%\begin{subequations}   
%    \label{eq:lim_omega_n_def}
%    \begin{IEEEeqnarray}{rCl}
%        \lim_{n \rightarrow \infty} \omega_{n} &=& 0, \\  
%          \lim_{n \rightarrow \infty}\left( \omega_{n}\sqrt{n} -\log n\right) &=& \infty,
%    \end{IEEEeqnarray}
%\end{subequations}
%%\eqref{eq:lim_omega_n_def}, and for each $t \in \mathcal{T}$ let $\rho_{1, t}, \rho_{2, t} \in \mathbb{R}_0^+$.
%Then, there  exists a sequence of encoding and decoding functions $\{(\varphi_1^{(n)}, \varphi_2^{(n)}, \phi_1^{(n)}, g_0^{(n)}, g_1^{(n)})\}_n$  so that for any $\epsilon >0$ and sufficiently large blocklengths $n$ the following two conditions hold:  
%\begin{IEEEeqnarray}{rCl}
% \lim_{n \rightarrow \infty} P_{e}  &\leq & \epsilon, \\
% \lim_{n \rightarrow \infty} \delta_{n,w_3} &\leq &  \epsilon \qquad \forall w_3 \in \mathcal{M}_3,
% \end{IEEEeqnarray}
% and the  message sizes $M_1, M_2, M_3$  and key size $K_1, K_2$ satisfy
 \begin{IEEEeqnarray}{rCl}
 \!\!\!\!\!\!\!\!\!\!\!\log(M_1) &=& (1-\xi_2) \omega_n \sqrt{n} \mathbb{E}_{P_{TX_3}} \left[ \rho_{1,T} D_{Y}^{(1)}(X_3) \right], \label{eq:th_1_log_m1} \\
\!\!\!\!\!\!\!\!\!\!\!\log(M_2) &=& (1-\xi_3) \omega_n \sqrt{n} \mathbb{E}_{P_{TX_3}} \left[ \rho_{2,T} D_{Y}^{(2)}(X_3) \right], \label{eq:th_1_log_m2}\\
 \!\!\!\!\!\!\!\!\!\!\!\log(M_3) &=& (1-\xi_4) n I(X_3;Y \mid X_1=0, X_2=0, T),\label{eq:th_1_log_m3} \\
\!\!\!\!\log(K_1K_2) &=& (1-\xi_5) \omega_{n}\sqrt{n} \mathbb{E}_{P_{TX_3}}  \left[ \sum_{k=1}^{2}\rho_{k,T} D_{Z-Y}^{(k)}(X_3) \right] \nonumber \\ \label{eq:th_1_log_k1_k2}
\end{IEEEeqnarray} 
%  \begin{figure*}
%     \begin{IEEEeqnarray}{rCl}
%  \log(K_1K_2) &=& (1-\xi_4) \omega_{n}\sqrt{n} \mathbb{E}_{P_{TX_3}}  \left[ \rho_{1,T} \left( D_{Z}^{(1)}(X_3) - D_{Y}^{(1)}(X_3) \right) + \rho_{2,T} \left( D_{Z}^{(2)}(X_3) - D_{Y}^{(2)}(X_3)) \right) \right].
%     \end{IEEEeqnarray}
%     \hrule 
% \end{figure*}
for  some small positive numbers $\xi_1,\xi_2, \xi_3, \xi_4 ,\xi_5\in (0,1)$ and the pmf $P_{TX_3}$ defined as:
\begin{equation}
P_{TX_3}(t, x_3) = \frac{n_t}{n} \cdot P_{X_3,t}(x_3),
\end{equation}

\end{theorem}
\begin{IEEEproof}
See Section~\ref{sec:coding}.
\end{IEEEproof}


The logarithmic scalings of the covert-message sizes $M_1$ and $M_2$  are at most  square-root-$n$ scalings (because $\omega_n$ vanishes), indicating that the number of covert bits that can be transmitted is only in the order of square-root-$n$ and not linear in $n$. For the logarithmic scaling of the noncovert-message sizes we have the usual linear-in-$n$ scaling. Communication of covert messages is thus of zero-rate while non-covert messages are communicated at standard  positive rates. 

The key and covert-message square-root-scalings all depend on the vanishing sequence $\omega_n$. Increasing $\omega_n$ proportionally-increases the permissible covert-message size but also quadratically increases the average divergence at the warden. To eliminate this dependence, we normalize the covert-message rates by the square-root of the average warden-divergence. We are thus interested in the following asymptotic (square-root) message and key rates: 
\begin{IEEEeqnarray}{rCl}
r_1 & :=& \lim_{n\to \infty} \frac{\log( M_1)}{\sqrt{\frac{n}{M_3} \sum_{w_3=1}^{M_3} \delta_{n, w_3} }} \\ 
r_2 & :=& \lim_{n\to \infty} \frac{\log(M_2)}{\sqrt{\frac{n}{M_3} \sum_{w_3=1}^{M_3} \delta_{n, w_3} }} \\ 
r_3 & :=& \lim_{n\to \infty} \frac{\log( M_3)}{n}  \\ 
k &:=&  \lim_{n\to \infty} \frac{\log (K_1 K_2)}{\sqrt{\frac{n}{M_3} \sum_{w_3=1}^{M_3} \delta_{n, w_3} }}. 
\end{IEEEeqnarray}
%Notice that the scaling of the number of covert messages bits $\log(M_1)$ and $\log(M_2)$ are not the usual scaling as is the case for the non-covert message bits $\log(M_3)$. In particular, covert communication takes place in a zero rate regime, and one cannot send more than $\mathcal{O}(\sqrt{n})$ bits to remain covert, motivating normalisation with $\sqrt{n}$. We further normalize by the average of the covertness constraints as this has a direct impact on the rate.
%For any pair $(x_3, t) \in \mathcal{X}_3 \times \mathcal{T}$ and non-negative real values $\rho_{1, t}, \rho_{2, t} \in \mathbb{R}_0^+$, where $\mathcal{T}$ is the time set, we define:

%The first one being the mixture output distribution and the second one the output distribution when the non-covert user is the only one communicating.
%% THEOREM 2 ASYMP ANALYSIS %%%%%%%%%%%%%%%%%%%%%%%%%%
We then obtain the following asymptotic capacity result for our setup with mixed covert and non-covert users. 
\begin{theorem}
\label{th:asymp_result}
There  exists a sequence of encodings and decodings with\begin{IEEEeqnarray}{rCl}
 \lim_{n \rightarrow \infty} P_{ei}  &=& 0, \qquad \forall i\in \{0,1\}, \\
 \lim_{n \rightarrow \infty} \delta_{n,w_3} &=& 0, \qquad \forall w_3 \in \mathcal{M}_3,
 \end{IEEEeqnarray}
 if, and only if, 
\begin{IEEEeqnarray}{rCl}
  r_1 
  &\leq& \sqrt{2} \frac{\mathbb{E}_{P_{TX_3}} \left[ \rho_{1,T} D_{Y}^{(1)}(X_3) \right]}{\sqrt{\mathbb{E}_{P_{TX_3}} \left[ \left( \rho_{1,T} + \rho_{2,T} \right)^2 \chi^2(\bm{\rho}_T, X_3) \right]}}\label{eq:asymp1}, \\
% \log(M_2}
 r_2 &\leq& \sqrt{2} \frac{\mathbb{E}_{P_{TX_3}} \left[ \rho_{2,T} D_{Y}^{(2)}(X_3) \right]}{\sqrt{\mathbb{E}_{P_{TX_3}} \left[ \left( \rho_{1,T} + \rho_{2,T} \right)^2 \chi^2(\bm{\rho}_T, X_3) \right]}}\label{eq:asymp2},\\[1.2ex]
 r_3 &\leq&  \mathbb{I}(X_3;Y \mid X_1=0,X_2=0,T)\label{eq:asymp3}, \\[1.2ex]
 k  &\geq& \sqrt{2} \frac{\mathbb{E}_{P_{TX_3}}  \left[ \sum_{k=1}^{2}\rho_{k,T} D_{Z-Y}^{(k)}(X_3) \right]} {\sqrt{\mathbb{E}_{P_{TX_3}} \left[ \left( \rho_{1,T} + \rho_{2,T} \right)^2 \chi^2(\bm{\rho}_T, X_3) \right]}},\label{eq:asympkey}
\end{IEEEeqnarray}
for some pmf $P_{X_3T}$ and parameters $\{\rho_{1,t},\rho_{2,t}\}_{t=1}^5$.
\end{theorem}
\begin{IEEEproof}
% See the following Section~\ref{sec:coding}.
Achievability follows directly from Theorem~\ref{main_theorem}. The converse is omitted due to lack of space.
\end{IEEEproof}
\subsection{Numerical examples}
\label{sec:simulations}
Consider binary input alphabets at all the users, i.e. $\mathcal{X}_1=\mathcal{X}_2=\mathcal{X}_3=\{0,1\}$ and channels (where rows indicate pairs $(x_1,x_2,x_3)$ in lexicographic order and columns the six $y$- or $z$-values)
\begin{subequations}\label{eq:channels}
    \begin{IEEEeqnarray}{rCl}
        W_{Y \mid X_1X_2X_3}=\begin{bmatrix}
            0.01 & 0.26 & 0.02 & 0.28 & 0.18 &  0.25 \\
            0.12 & 0.36 & 0.29 & 0.06 & 0.11 &  0.06 \\
            0.17 & 0.14 & 0.25 & 0.10 & 0.13 &  0.21 \\
            0.05 & 0.15 & 0.31 & 0.28 & 0.01 &  0.20 \\
            0.08 & 0.39 & 0.02 & 0.25 & 0.18 &  0.08 \\
            0.05 & 0.21 & 0.13 & 0.28 & 0.03 &  0.30 \\
            0.15 & 0.05 & 0.10 & 0.17 & 0.33 &  0.20 \\
            0.05 & 0.25 & 0.10 & 0.20 & 0.10 &  0.30 
        \end{bmatrix}, \nonumber \\
    \end{IEEEeqnarray}
    \begin{IEEEeqnarray}{rCl}
        \Gamma_{Z \mid X_1X_2X_3}= \begin{bmatrix}
            0.15 & 0.11 & 0.57 & 0.01 & 0.06 & 0.10 \\
            0.15 & 0.41 & 0.12 & 0.15 & 0.06 & 0.11 \\
            0.23 & 0.02 & 0.01 & 0.48 & 0.10 & 0.16 \\
            0.14 & 0.17 & 0.21 & 0.12 & 0.24 & 0.12 \\
            0.01 & 0.12 & 0.19 & 0.15 & 0.19 & 0.34 \\
            0.10 & 0.11 & 0.15 & 0.14 & 0.18 & 0.32 \\
            0.05 & 0.15 & 0.15 & 0.20 & 0.10 &  0.35 \\
            0.10 & 0.10 & 0.27 & 0.13 & 0.20 &  0.20
        \end{bmatrix}. \nonumber \\
    \end{IEEEeqnarray}
\end{subequations}
% \begin{subequations}\label{eq:channels}
%     \begin{IEEEeqnarray}{rCl}
%         &&\lefteqn{W_{Y \mid X_1X_2X_3}=} \nonumber \\
%         && \begin{bmatrix}
%             0.0089 & 0.2666 & 0.0040 & 0.2805 & 0.1948 &  0.2452 \\
%             0.1162 & 0.3655 & 0.2891 & 0.0553 & 0.1071 &  0.0668 \\
%             0.1705 & 0.1418 & 0.2525 & 0.0257 & 0.1328 &  0.2767 \\
%             0.0079 & 0.1471 & 0.3133 & 0.2759 & 0.0038 &  0.2520 \\
%             0.0821 & 0.3956 & 0.0161 & 0.2547 & 0.1895 &  0.0619 \\
%             0.0510 & 0.2062 & 0.1389 & 0.2814 & 0.0179 &  0.3045 
%         \end{bmatrix}, \nonumber \\
%     \end{IEEEeqnarray}
% \end{subequations}
% \begin{subequations}\label{eq:channels}
%     \begin{IEEEeqnarray}{rCl}
%         &&\lefteqn{W_{Z \mid X_1X_2X_3}=} \nonumber \\
%         && \begin{bmatrix}
%             0.1559 & 0.1123 & 0.5683 & 0.0067 & 0.0545 & 0.1023 \\
%             0.1493 & 0.4114 & 0.1206 & 0.1514 & 0.0601 & 0.1072 \\
%             0.2299 & 0.0195 & 0.0094 & 0.4777 & 0.1063 & 0.1572 \\
%             0.1413 & 0.1672 & 0.2081 & 0.1177 & 0.2389 & 0.1267 \\
%             0.0034 & 0.1171 & 0.1963 & 0.1493 & 0.1930 & 0.3409 \\
%             0.0933 & 0.1089 & 0.1509 & 0.1372 & 0.1829 & 0.3267 
%         \end{bmatrix}. \nonumber \\
%     \end{IEEEeqnarray}
% \end{subequations}
% \highlight{Add the figures and update the comments here later! Say also why intuitively timesharing is beneficial, use experiment of T=1 vs T=2. Or maybe include this after the coding scheme and state that the users cooperate in a statistical sens through the timesharing r.v.}\\
% Notice that these channels satisfy Conditions \eqref{eq:channel_conditions}.
% Consider the channel laws in \eqref{eq:channels}.
Figure~\ref{fig:simulation_time_sharing_beneficial}, illustrates the rate-region in Theorem~\ref{th:asymp_result} under the additional constraint that the  secret-key rate be smaller than $k\leq 0.8$ (solid red curve) and the corresponding reduced rate-region when one further imposes that $T=1$ deterministically, i.e., when in our scheme communication takes place only over a single phase. This juxtaposition clearly demonstrates the enhancement in capacity, i.e., achievable square-root rates, when the users  can communicate  over different phases and using different codes in the various phases. 
The forthcoming discussion  delves into the rationale underlying this enhancement.
% We shall now give some intuitions about why this is the case.
% In fact, there is no direct cooperation between the three users.
% Nevertheless, they all share a known timesharing sequence $t^n$ that they use to construct their respective codewords.
% Thus, the users are cooperating in a statistical sens, which allows the covert users 1 and 2 to choose their power values ($\rho_{1,t}$ and $\rho_{2,t}$) accordingly and send more or less $1$-symbols.

%Although the three users do not directly cooperate, they do share a common, predetermined time-sharing sequence denoted as $t^n$, which they use to generate their respective codewords. 
%This shared time-sharing sequence engenders a form of statistical cooperation among the users, thereby enabling covert Users 1 and 2 to dynamically adjust their power allocation parameters, denoted as $\rho_{1,t}$ and $\rho_{2,t}$ (at each time instance $t \in \mathcal{T}$), and consequently transmit varying numbers of $1$-symbols.
%More specifically, communication of the non-covert user influences the channel conditions at the different phases of communication, at times facilitating covert users to communicate at higher rates, i.e. when the non-covert user creates less favorable channels with respect to the warden, and conversely, when it generates favorable channels at other times.

Furthermore, the conclusions articulated in this discourse can be substantiated by the empirical findings as depicted in Figure~\ref{fig:non_covert_improves_covert_capacity}. This graphical representation delineates the maximum covert rate $r_2$, as a function of the secret-key rate $k$. 
The optimization process is conducted over the probability distribution $P_{X_3}$, yielding the red curve. In contrast, the dashed blue curve and the dash-dotted black curve illustrate the corresponding performance when the non-covert user sends a constant symbol, specifically $X_3=0$ and $X_3=1$, respectively.
It is evident from this empirical evidence that non-constant channel inputs at User 3, represented by $X_3$, deliver superior performance compared to the two constant channel inputs.
In this sens, the presence of the non-covert user within the system effectively amplifies the covert capacity of the covert user 2.
% These conclusions can be further supported by the simulation in Figure~\ref{fig:non_covert_improves_covert_capacity}, which illustrates the largest possible covert rate $r_2$ in function of the secret-key rate $k$, when one optimizes over $P_{X_3}$,  (red curve) and when the non-covert user sends the constant symbol $X_3=0$ (dashed blue curve) or $X_3=1$ (dash-dotted black curve). This shows that non-constant channel inputs $X_3$ at User 3 achieve better performance than any of the two constant channel inputs. In this sense, the presence of User 3 in the system actually increases the covert capacity of the covert User 2.

Figure~\ref{fig:simulation_r2_vs_r3_for_different_rate_r1} illustrates the rate-region at different rates $r_1$ for the covert User 1, showcasing the trade-offs between the three users.
% Considering the inputs $X_3^n$ a state sequence that influences the channel, above observations imply that a state-dependent channel can have higher covert rate for a given secret-key rate then any of the marginal channels that result when one fixes the channel state. State-dependent covert-communication was also considered in \cite{ligong_csi_uncertainty_tx, bloch_keyless_csi, bloch_keyless_csi_journal, bloch_coop_jammer}.

\input{plots/used/timesharing_beneficial}
\input{plots/used/non_covert_improves_covert_capacity}
\input{plots/used/r1_vs_r2_vs_r3}
% \input{plots/used/T=2vsT=1}
% \input{plots/used/timesharing_r1=0.15}

% Figure~\ref{fig:simulation_3D} illustrates the rate-region $(r_1,r_2,r_3)$ in Theorem~\ref{th:asymp_result} for the channels in \eqref{eq:channels} and secret-key rate $k\leq 0.8$. 
% \begin{figure}[!h]
%     \centering
%     \includegraphics[width=9cm]{figures/contour_plot_3D.pdf}    
%     \caption{Rate-region $(r_1,r_2,r_3)$  for the channels in \eqref{eq:channels} and secret-key rate $k\leq 0.8$.}
%     \label{fig:simulation_3D}
% \end{figure}

% For a better visualization of the rate-region, we present the relationships in 2D. In particular, Figure~\ref{fig:simulation_r1_vs_r2} shows the rate-region $(r_1,r_2,r_3=0)$. Notice that in this scenario, we recover the results presented in \cite{bloch_k_users_mac} with a scheme that includes time-sharing. In both Figures~\ref{fig:simulation_r1_vs_r3} and \ref{fig:simulation_r2_vs_r3}, we illustrate the rate-regions $(r_1,r_2=0,r_3)$ and $(r_1=0,r_2,r_3)$ respectively. In this scenario, we recover the results we presented in \cite{ours_first}.
\subsection{Discussion and Remarks}
Theorem~\ref{th:asymp_result} allows for a pleasing intuitive discussion with respect to the various information quantities involved. In particular, \eqref{eq:asymp1} and \eqref{eq:asymp2} suggests that the covert rate depends on the ability of the legitimate receiver to distinguish the two input symbols, normalized by the ability of the warden into distinguishing them. Moreover, in view of Theorem~\ref{th:asymp_result}, few remarks are in order.
% \begin{remark}
% Notice that the tuple $\bm{\rho_t}$ represents how we allocate the number of $1$ symbols for each of the covert users at each time instance $t \in \mathcal{T}$. 
% Lemma~\ref{lemma_1_asymptotics} suggests that for each non-covert symbol $x_3 \in \mathcal{X}_3$, the chi-square distance $\chi_n^2(\bm{\rho}_t, x_3)$ controls covertness and is common to the two covert users' rates as communication of each of them jointly affects the covertness constraint.
% \end{remark}
\begin{remark}
Whenever the nominator of \eqref{eq:asympkey} is negative for any choice of the pmf $P_{TX_3}$, the condition \eqref{eq:asympkey} is always satisfied and no secret key is required for covert communication. This connects with the wiretap channel condition as the channel of the legitimate receiver becomes better than the one of the attacker.
\end{remark}
\smallskip
\begin{remark}
For $\mathcal{X}_2 = \{x_2\}$ a singleton, we recover the result in \cite{ours_first} for the channel $W_{Y|X_1X_2X_3}(\cdot|\cdot,x_2,\cdot)$. In this case, and for all $t \in \mathcal{T}$, upon defining $\epsilon_t=\rho_{1,t}$ and setting $\rho_{2,t}=0$, it suffices to choose $|\mathcal{T}|=2$ and the expression in \eqref{eq:asymp1}, \eqref{eq:asymp3} remains unchanged, while \eqref{eq:asympkey} further simplifies to match the secret-key rate in \cite{ours_first}.
\end{remark}
\smallskip
\begin{remark}
For $\mathcal{X}_3 = \{x_3\}$ and $\mathcal{T} = \{t\}$ both singletons, we recover the findings of \cite{bloch_keyless} for the channel $W_{Y|X_1X_2X_3}(\cdot|\cdot,\cdot,x_3)$. This alignment is contingent on two assumptions made in \cite{bloch_keyless}. In particular, assuming that the legitimate receiver channel is better than the warden's channel (so that no secret key is needed for covertness). Additionally, by assuming that $\rho_{1,t}+\rho_{2,t}=1$, the expressions in \eqref{eq:asymp1} and \eqref{eq:asymp2} matches those presented in \cite{bloch_keyless}.
\end{remark}
\smallskip
\begin{remark}
For $\mathcal{X}_2 = \{x_2\}$ and $\mathcal{X}_3 = \{x_3\}$ both singletons, we recover the results in \cite{bloch_first} for the channel $W_{Y|X_1X_2X_3}(\cdot|\cdot,x_2,x_3)$. In this case it suffices to choose $T$ deterministic, i.e., $|\mathcal{T}|=1$ and setting $\rho_{2,t}=0$ so that the expression in \eqref{eq:asymp1}, \eqref{eq:asympkey} further simplify in the sense that the $\rho_{1,T}$-terms in the fraction can be reduced and the final expression does not depend on $\rho_{1,T}$ anymore.
\end{remark}

==> contents/conclusion.tex <==
\section{Summary and Discussion}
\label{sec:conclusion}
In this work, we established the fundamental limits of a communication system comprising two covert users and one a non-covert user, all communicating to the same receiver, which also shares a common secret-key with the covert users of a given secret-key rate. 
Our findings illuminate an intricate interplay among three pivotal quantities: the covert users' rates, the non-covert users' rate and the secret-key rate.
Importantly, our results emphasize the necessity of a coded time-sharing strategy among these users, akin to multi-access scenarios without covert constraints.
Moreover, our results also highlights that the presence of the non-covert user can potentially improve the covert-capacity under a stringent key-rate constraint.

While our results are for MACs with a two coverts and one non-covert users, extensions to multiple users with arbitrary finite alphabet (not only binary) for the covert users seems feasible and is part of ongoing research. 
% Other interesting research direction include covert communication over the interference channel with the presence of non-covert users as well as transmission of channels with
% Additionally, our results suggests that having a non-covert user can potentially improve covert capacity under stringent key-rate constraints.
% Our ongoing work explores extensions to scenarios with multiple users using arbitrary finite alphabets, beyond binary encoding for covert users.

==> contents/converse.tex <==
% \subsubsection{Converse Proof} \label{sec:converse}
% \highlight{to be discussed...}

==> contents/intro.tex <==
\section{Introduction}
\label{section:introduction}
\IEEEPARstart{G}{}uaranteeing privacy and security of Internet of Things (IoT) communication is a major challenge~\cite{iot_security_survey} due to the broadcast nature of wireless commuunication. 
% Physical Layer Security (PLS), leverage information-theoretic techniques and the characteristics of wireless channels to enhance the security of communications and make it harder for attackers to intercept or decipher transmitted data.
A recent and promising technique within physical layer security is covert communication, which involves conveying information with minimal probability of detection by other users, adversaries, or network monitoring nodes.
Such communication setups are relevant in future IoT and sensor networks.
%as they allow one to add a layer of privacy on top of a private network.
% For instance in healthcare applications, sensors in a hospital may transmit sensitive data and this data should be reliably decoded by authorized devices while staying undetectable by any unauthorized one.
For instance in healthcare applications, encryption and decryption of complex and voluminous sensitive data such as Electrocardiogram data can be time-consuming and resource-intensive, which can be a concern for resource-constrained devices or environments.
% for some sensitive data such as Electrocardiogram (ECG) data, it might be more practical to send the data covertly rather than encrypting it at the edge sensor. 
% In fact ECG data is often voluminous and complex. 
% It contains a high number of data points, which can make encryption and decryption processes time-consuming and resource-intensive. 
% In particular, strong encryption algorithms can consume significant computational resources, which can be a concern for resource-constrained devices or environments.
% Moreover, the metadata associated with the data that can potentially reveal sensitive information. In the case of ECG data, even if it is encrypted, an observer might still be able to infer certain information based on the timing and frequency of data transmissions. They may deduce when a patient is receiving treatment, experiencing health issues, or even the general patterns of their daily life.
% Furthermore, analyzing patterns in the encrypted data, such as packet size and transmission timing, can sometimes provide informations about the nature of the data being transmitted. In the case of ECG data, certain patterns might be recognizable even if the content itself is encrypted.\\
% require undetectability which is stronger than encryption.
To maintain a covert communication, users must remain silent for most of the time and transmit a small number of information bits. 
In the context of IoT, such a small number of bits per device suffices in many applications, and as such, covert communication seems an adequate approach to ensure secure IoT communication. Compared to conventional cryptographic algorithms, this communication scheme is energy-efficient, which is particularly beneficial for IoT devices that have limited battery life. 
The pioneering work \cite{bash_first} characterized the fundamental limits of covert communications over AWGN channels. It showed that it is possible to communicate covertly as long as the message is subject the so-called \emph{square-root law}, i.e., the number of  communicated bits scales like $\mathcal{O}(\sqrt{n})$, for  $n$  indicating the number of channel uses. %The \emph{covert capacity} defines then the optimal scaling in $\mathcal{O}(\sqrt{n})$. 
The findings of a number of recent works~\cite{bash_first, bash_p2p, bloch_first, ligong_first}, made the \emph{square-root law} become the de-facto standard limit of covert communication for most, if not all, scenarios and channels.
% In particular, it has been recently established in various works  \cite{bash_first, bash_p2p, bloch_first, ligong_first} that the fundamental limits of covert communication is indeed characterized by this  \emph{square-root law}. %,  for example for the point-to-point Discrete Memoryless Channel (DMC)   and AWGN channels. 
%Many works investigated then different covert setups over different channels satisfying this \emph{square-root rate} limit. In particular, \cite{bloch_first} and  \cite{ligong_first} derived the fundamental limits for classical point-to-point channels. 
% While \cite{ligong_first} assumed the existence of a sufficiently large secret key allowing covertness, \cite{bloch_first} derived the exact growth rate of this secret key and established  conditions where it is not needed. These results were also extended to keyless  setups over binary symmetric channels (BSCs) \cite{che_keyless} and over Multiple Access Channels (MACs) \cite{bloch_k_users_mac}, and to asymptotically keyless setups \cite{bloch_asymp_keyless}. %For channels with multiple users, \cite{bloch_first} extended their work on point-to-point channels and characterized the covert capacity for a $K$-user MAC \cite{ bloch_k_users_mac}. 
Higher covert-rates than indicated by the \emph{square-root law} were shown to be achievable in scenarios where the warden has uncertainty about the channel statistics \cite{che_uncertainty, ligong_csi_uncertainty_tx, bloch_keyless_csi, bloch_keyless_csi_journal} or in the presence of a jammer \cite{bash_uninformed_jammer, shmuel_multi_antennas_jammer, bloch_coop_jammer}.
More closely related  to this paper are \cite{bloch_journal_embedding_broadcast, ligong_broadcast, sang_multiple_overt_superposition_covert_on_overt, sang_noma_multiple_overt_superposition_covert_on_overt, ours_first} which consider extensions to Broadcast Channels (BCs) and Multiple Access Channels (MACs).
% In particular, \cite{bloch_journal_embedding_broadcast} characterized the limits of covert communication over a BC when the transmitter sends a common  non-covert message to two receivers and a covert message to only one of them by  embedding the covert codeword into the non-covert codeword. 
% Using superposition coding, they jointly design a code for the secret message and the common message. 
% In contrast, \cite{ligong_broadcast} studied the same problem under a stronger assumption, i.e. the codebook of the common message is fixed, which gives less freedom to the transmitter in order to find the common message that is the best for superposition. 
% Furthermore, \cite{sang_multiple_overt_superposition_covert_on_overt, sang_noma_multiple_overt_superposition_covert_on_overt} extended this setup to the case where many non-covert users are communicating and the superimposing is done on one of the common message codewords. Subsequently, they showed that under the assumption that the non-covert codeword that is used for the superposition is not decoded by the warden, covert communication is possible and the probability of detection can converge faster to 0 when the number of non-covert users increases.\\
% Extensions to scenarios with a fixed  codebook for the common message or with several receivers were presented in  \cite{ligong_broadcast} \cite{sang_multiple_overt_superposition_covert_on_overt, sang_noma_multiple_overt_superposition_covert_on_overt}. These works identified the dependence of the amount of covert bits on the channel parameters and showed that the probability of detection of the warden can vanish faster when increasing the number of non-covert users.
% The results of \cite{sang_multiple_overt_superposition_covert_on_overt, sang_noma_multiple_overt_superposition_covert_on_overt} showed that the probability of detection can converge faster to 0 when the number of non-covert users increases. In our work, a similar conclusion was derived.

This paper is a follow up for our recent results on covert communication~\cite{ours_first} where the objective is to generalize to other setups than the ones previously studied. 
Precisely, as a first step toward the generalization, we consider in this work a Discrete Memoryless Multiple Access Channel (DM-MAC) with three users communicating with a legitimate receiver. 
More specifically, sharing a secret key with this receiver, both User 1 and User 2 wishes to communicate covertly without being detected by an external warden. 
In contrast, User 3 transmits a non-covert message to the same legitimate receiver.
The covertness constraint imposes in this scenario that the communication of all users must resemble communication of the non-covert user rather than pure noise as in standard setups~\cite{bash_first, bloch_first, ligong_first, bloch_k_users_mac}. 
We establish the fundamental limits on the set of achievable tuples of non-covert rate, covert rates, and secret-key rates.
Our setup requires non-trivial steps as it was the case in our recent work~\cite{ours_first} from which we borrowed proof techniques.
% Compared to the previous related results \cite{bloch_first, ligong_first, ligong_broadcast, bloch_journal_embedding_broadcast, bloch_k_users_mac}, our setup required extra non-trivial steps especially in the asymptotic analysis and converse proof. Throughout our proofs, we borrowed techniques that we used in our recent work~\cite{ours_first}.

We show through numerical examples that coded time-sharing improves the covert user's capacity under a secret-key rate constraint. 
Moreover, we observe a tradeoff between the rates of the non-covert and covert users respectively, which illustrates the dependence of the covert rate on the channel parameters, emphasizing the influence of the non-covert codewords on the achievable covert rate. We also show that the covert user's rate  can be improved in the presence of a non-covert user. 
These conclusions, along with the ones made in \cite{ sang_multiple_overt_superposition_covert_on_overt, sang_noma_multiple_overt_superposition_covert_on_overt}, which showed that the probability of detection  vanishes faster when one increases the number of non-covert users, suggests that covert communication can be enhanced via the presence of non-covert users. 
The proofs are omitted for consistency and due to lack of space.
% \textbf{The proofs are omitted for consistency and due to lack of space. Interested readers are referred to~\cite{ours_two_covert_one_non_covert}.}

\section{Notation}
% \emph{Notation}: 
In this paper, we follow standard information theory notations. 
We use $\mathbb{I}(\cdot;\cdot)$ for the mutual information of random variables.
We note by $\left| \mathcal{S} \right|$ the cardinality of a set $\mathcal{S}$. 
The set $[|1,N|]$ denotes the set of positive integers between $1$ and $N$.
Random variables are denoted by upper case letters (e.g., X), while their realizations are denoted by lowercase (e.g. x). We write $X^{n}$ and $x^{n}$ for the tuples $(X_1,\ldots, X_n)$ and $(x_1,\ldots, x_n)$, respectively, for any positive integer $n > 0$. 
For a distribution $P$ on $\mathcal{X}$, we note its product distribution on $\mathcal{X}^{n}$ by $P^{\otimes n}(x^{n}) = \prod_{i=1}^{n} P(x_{i})$. 
For two distributions $P$ and $Q$ on $\mathcal{X}$, $D(P\|Q)=\sum_{x \in \mathcal{X}} P(x)\log(\frac{P(x)}{Q(x)})$ is the relative entropy.
The type of a sequence $x^n\in\mathcal{X}^n$ is defined as $\pi_{x^n}(a) =  \left| \{t\colon x_t=a \}\right| / n$ and the strongly-typical set $\mathcal{T}_{\mu}^{(n)}(P_{X})$ \cite[Definition 2.8]{Csiszarbook} is the subset of sequences $x^n\in\mathcal{X}^n$ that satisfy $|\pi_{x^n}(a)- P_X(x)|  \leq \mu$ for all $a\in\mathcal{X}$ and whenever $P_X(x)=0$ then also $\pi_{x^n}(a)=0$. We further abbreviate \emph{probability mass function} by \emph{pmf}.
The logarithm and exponential functions are in base $e$ and we define $0 \log(0) = 0$. 
We define $\mathcal{X}_1,\mathcal{X}_2$ and $\mathcal{X}_3$ to be the input alphabets of user 1, user 2 and user 3 respectively. 




==> contents/main_result_and_simulation.tex <==
\section{Main Results}
Our main results are an achievability result for finite blocklengths and a converse that asymptotically matches this achievability analysis.
For brevity of the description, we omit the details of the proofs that are same to that of \cite{ours_first}. Instead, we
provide comments and intuitions to help understanding.
% Following our previous work \cite{ours_first}, we assume that for any $x_3 \in \mathcal{X}_3$ the channel satisfies the following three conditions:
% \begin{subequations}\label{eq:channel_conditions}
% \begin{IEEEeqnarray}{rCl}
% W_{01x_3}(\cdot) & \ll & W_{00x_3}(\cdot), \\
% W_{01x_3}(\cdot) & \neq & W_{00x_3}(\cdot), \\
% W_{10x_3}(\cdot) & \ll & W_{00x_3}(\cdot), \\
% W_{10x_3}(\cdot) & \neq & W_{00x_3}(\cdot), \\
% \Gamma_{01x_3}(\cdot) & \ll & \Gamma_{00x_3}(\cdot), \\
% \Gamma_{01x_3}(\cdot) & \neq & \Gamma_{00x_3}(\cdot), \\
% \Gamma_{10x_3}(\cdot) & \ll & \Gamma_{00x_3}(\cdot), \\
% \Gamma_{10x_3}(\cdot) & \neq & \Gamma_{00x_3}(\cdot).
% \end{IEEEeqnarray}
% \end{subequations}
% Notice that intuitively, these assumptions exclude cases where covert communication is either trivial, (i.e. when the warden output distributions are the same whatever the input is) or impossible, (i.e. when the legitimate receiver cannot distinguish the two outputs).



==> contents/problem_statement.tex <==
\section{Problem statement}
\label{sec:problem_statement}
\begin{figure}[t!]
   \centering
   \includegraphics[scale=0.625]{figures/ICC2023_setup_2_covert_1non_covert_without_naming_on_dec_messages.pdf}
   \caption{Multi-access communication where communication of User 1 and User 2 has to remain undetectable to an external warden. The messages $W_1$ and $W_2$ are the covert messages, while $W_3$ is the non covert message.}
   \label{fig:setup}
\end{figure}
\label{section:problem_setup_and_main_result}
Consider the three-user single-receiver setup in Figure \ref{fig:setup} where an external warden should not be able to detect communication from 
 Users 1 and 2. Communication from User 3 has no detectability constraints, and we can even allow the warden to know its transmitted message.\footnote{Providing the warden with the  message of User 3 makes the warden only stronger. The rates that are achievable under such a strong warden remain also achievable under weaker assumptions on the warden.}. 
We model our setup using two hypotheses $\mathcal{H}=0$ and $\mathcal{H}=1$, where under $\mathcal{H}=0$ only User 3 is transmitting  while under $\mathcal{H}=1$ all three users transmit, and the warden wishes to guess the true hypothesis. Details are as follows.
For simplicity of illustration, we assume that Users 1 and 2 produce inputs in the binary alphabet $\mathcal{X}_1=\mathcal{X}_2=\{0,1\}$ and we consider that $0$ is the "off-symbol", i.e. the symbol transmitted by Users 1 and 2 under $\mathcal{H}=0$. User~3's input alphabet $\mathcal{X}_3$ is finite but arbitrary otherwise. 
The legitimate receiver and the warden observe channel outputs in the finite alphabets $\mathcal{Y}$ and $\mathcal{Z}$. 
% These outputs are produced by a discrete and memoryless interference channel with transition laws $W_{Y|X_1X_2X_3}$ and $\Gamma_{Z|X_1X_2X_3}$ respectively, see Figure~\ref{fig:setup}. 
Define the message and key sets 
\begin{IEEEeqnarray}{rCl}
\mathcal{M}_{i} &\triangleq& \{1, \ldots, M_{i} \}, \quad \forall i \in \{1,2,3\},\\
\mathcal{K}_j & \triangleq & \{1,\ldots, K_j\}, \quad \forall j \in \{1,2\},
\end{IEEEeqnarray}
% \begin{IEEEeqnarray}{rCl}
% \mathcal{M}_{1} &\triangleq& \{1, \ldots, M_{1} \}\\
% \mathcal{M}_{2} &\triangleq& \{1, \ldots, M_{2} \}\\
% \mathcal{M}_{3} &\triangleq& \{1, \ldots, M_{3} \}\\
% \mathcal{K}_1 & \triangleq & \{1,\ldots, K_1\}\\
% \mathcal{K}_2 & \triangleq & \{1,\ldots, K_2\}
% \end{IEEEeqnarray}
for given numbers $M_1$,  $M_2$, $M_3$, $K_1$, and $K_2$ and let the messages $W_1$, $W_2$, $W_3$ and the keys $S_1$ and $S_2$ be independent of each others and uniform over $\mathcal{M}_1, \mathcal{M}_2$, $\mathcal{M}_{3}$, $\mathcal{K}_1$ and $\mathcal{K}_2$, respectively. 
The key $S_1$ is known to User 1 and to the legitimate receiver, while message $W_1$ is known  to User 1 only. 
Similarly, the key $S_2$ is known to User 2 and to the legitimate receiver and the message $W_2$ is known  to User 2 only. 
In contrast $W_3$ is known to User 3 and is given to the warden. \\
\textit{\underline{Under $\mathcal{H}=0$:}}\\
Users 1 and 2 send the all-zero sequences 
\begin{align}
X_1^n&=0^n,\\
X_2^n&=0^n,
\end{align} 
meaning that they are not communicating, whereas User 3 applies some  encoding function $x_1^{(n)}\colon \mathcal{M}_3 \to \mathcal{X}_3^n$ to its message $W_3$ and sends the resulting codeword 
\begin{equation}\label{eq:X3}
% X_3^n=x_3^n(W_3)
X_3^n=x_1^{(n)}(W_3)
\end{equation} over the channel.\\
\textit{\underline{Under $\mathcal{H}=1$:}}\\
User 1 applies some  encoding function $x_1^{(n)}\colon \mathcal{M}_1 \times \mathcal{K}_1\to \mathcal{X}_1^n$ to its message $W_1$ and the secret key $S_1$ and sends the resulting codeword 
\begin{equation}
% X_1^n=x_1^n(W_1,S_1)
X_1^n=x_1^{(n)}(W_1,S_1)
\end{equation} over the channel. 
Similarly, User 2 applies some encoding function $x_2^{(n)}\colon \mathcal{M}_2 \times \mathcal{K}_2\to \mathcal{X}_2^n$ to its message $W_2$ and the secret key $S_2$ and sends the resulting codeword 
\begin{equation}
% X_2^n=x_2^n(W_2,S_2)
X_2^n=x_2^{(n)}(W_2,S_2)
\end{equation} over the channel. 
User 3 constructs its channel inputs in the same way as before, see~\eqref{eq:X3}.
% since it is not inevitably 
User 3 can be unaware of whether $\mathcal{H}=0$ or $\mathcal{H}=1$. 
% For readability we will also write $x_1^n(w_1,s_1)$, $x_2^n(w_2,s_2)$ and $x_3^n(w_3)$ instead of $\varphi_1^{(n)}(w_1,s_1)$,  $\varphi_2^{(n)}(w_2,s_2)$ and $\phi_1^{(n)}(w_3)$.

The legitimate receiver,  which knows the hypothesis $\mathcal{H}$, decodes the desired messages $W_3$ (under $\mathcal{H}=0$) or  $(W_1,W_2,W_3)$ (under $\mathcal{H}=1$) based on its knowledge of the keys $(S_1,S_2)$ and its observed outputs $Y^n=(Y_1,\ldots, Y_n)$ which are generated by a discrete memoryless channel $W_{Y \mid X_1X_2X_3}$ from the input sequences $X_1^n, X_2^n, X_3^n$.
That means, if $X_1^n=x_1^n$, $X_2^n=x_2^n$, and $X_3^n=x_3^n$ then the $i$-th output symbol $Y_i$ is generated from the $i$-th inputs $x_{1,i}, x_{2,i}, x_{3,i}$ according to the conditional channel law $W_{Y \mid X_1X_2X_3}(\cdot \mid x_{1,i}, x_{2,i}, x_{3,i})$ for any $i \in \{1, \ldots, n\}$.
Therefore, under $\mathcal{H}=0$ it uses a decoding function $g_0^{(n)}\colon \mathcal{Y}^n \to \mathcal{M}_3$ to produce the single guess
\begin{equation}
\widehat{W}_3 = g_0^{(n)}( Y^n)
\end{equation}
and under $\mathcal{H}=1$ it uses a decoding function $g_1^{(n)}\colon \mathcal{Y}^n \times \mathcal{K}_1 \times \mathcal{K}_2 \to \mathcal{M}_1 \times  \mathcal{M}_2 \times  \mathcal{M}_3$ to produce the triple of guesses
\begin{equation}
(\widehat{W}_1,\widehat{W}_2, \widehat{W}_3) = g_1^{(n)}( Y^n, S_1, S_2). 
\end{equation}
% \begin{multline}
%     \label{eq:noma_u1}
%         \!\!\!u_1\Big(\frac{L^{UL}}{C_1^{\text{NOMA, UL}}}+T^{w}
%     \\ +\frac{L^{DL}}{\min(C_2^{\text{NOMA, DL}}, C_1^{\text{NOMA, DL}})} \\ + \frac{1}{\beta} \cdot \frac{L^{DL}}{C_1^{\text{NOMA, DL}}} + \frac{1}{\beta} \cdot \frac{L^{DL}}{C_2^{\text{NOMA, DL}}} \Big) \leq T^s
% \end{multline}
The performance of decoding associated with a tuple of encoding and decoding functions $(x_1^{(n)}, x_2^{(n)}, x_3^{(n)}, g_0^{(n)}, g_1^{(n)})$ is measured by the following error probabilities under the two hypotheses:
\begin{IEEEeqnarray}{rCl}
    P_{e0} & \triangleq & \Pr\left(\widehat{W}_3 \neq W_3 \Big| \mathcal{H}=0\right), \label{eq:prob2} \\
    % P_{e1} & \triangleq &\Pr\left(\widehat{W}_3 \neq W_3 \text{ or } \widehat{W}_{2} \neq W_{2} \text{ or } \widehat{W}_{1} \neq W_{1} \Big| \mathcal{H}=1\right). \nonumber\\ \label{eq:prob1}
    P_{e1} &\triangleq& \Pr\left(\bigcup_{i=1}^3 \widehat{W}_i \neq W_i \Big| \mathcal{H}=1\right). \label{eq:prob1}
\end{IEEEeqnarray}  
Furthermore, communication is subject to a covertness constraint at a warden, which besides message $W_3$, also observes channel outputs $Z^n$, which are generated from inputs $X_1^n, X_2^n, X_3^n$ according to an arbitrary but given discrete and memoryless channel law $\Gamma_{Z \mid X_1X_2X_3}$. 
By the uniform nature of the messages and the keys, for each $w_3\in \mathcal{M}_3$ and $W_3=w_3$, the warden's output distribution under $\mathcal{H}=1$ is thus given by
\begin{multline}
    \label{eq:def_Q_C_w3}
        \widehat{Q}_{\mathcal{C}, w_3}^{n}(z^{n}) \triangleq  \frac{1}{M_1M_2K_1K_2} \Bigg[ \sum_{(w_1,s_1)} \sum_{(w_2,s_2)} \\
        W^{\otimes n}_{Z|X_1X_2X_3} (z^n| x_1^n(w_1,s_1), x_2^n( w_2,s_2), x_3^n(w_3))\Bigg],
\end{multline}
% in \eqref{eq:def_Q_C_w3} on the top of next page
%  \begin{figure*}
% \begin{IEEEeqnarray}{rCl}
%     \label{eq:def_Q_C_w3}
%         \widehat{Q}_{\mathcal{C}, w_3}^{n}(z^{n}) &\triangleq&  \frac{1}{M_1M_2K_1K_2} \sum_{(w_1,s_1)} \sum_{(w_2,s_2)} W^{\otimes n}_{Z|X_1X_2X_3} (z^n| x_1^n(w_1,s_1), x_2^n( w_2,s_2), x_3^n(w_3)),
% \end{IEEEeqnarray}
%  \hrule \end{figure*}
and under $\mathcal{H}=0$, it is given by
\begin{IEEEeqnarray}{rCl}
W^{\otimes n}_{Z|X_1X_2X_3} (z^n| 0^n, 0^n, x_3^n(w_3)).
\end{IEEEeqnarray}
For any $w_3 \in \mathcal{M}_3$ we  define the covertness constraint as the divergence between these two distributions:
\begin{equation}
\label{eq:def_delta_n_w3}
\delta_{n,w_3}\triangleq \mathbb{D}\left(\widehat{Q}_{\mathcal{C}, w_3}^{n} \big\| W^{\otimes n}_{Z|X_1X_2X_3} ( \cdot | 0^n, 0^n, x_3^n(w_3))\right).
\end{equation}
The choice of this measure for covertness can be justified by its presence in \emph{Stein's Lemma} where it shows up as the error exponent of a binary hypothesis test. 
Standard arguments \cite{cover} can be used to relate this divergence to the warden's detection error probabilities.
Notice that our problem is multi-objective in the sens that we not only wish to have a reliable communication, i.e. vanishing error probabilities \eqref{eq:prob2} and \eqref{eq:prob1}, but we require also a vanishing  detectability capability \eqref{eq:def_delta_n_w3}. 
% This problem can be framed by the following definition:
% \begin{definition}
% A tuple $(r_1,r_2,r_3,k)$ is achievable if there exists a sequence (in the blocklength $n$)  of tuples $(M_1,M_2,M_3,K_1,$ $K_2)$ and encoding/decoding functions $(\varphi_1^{(n)}, \varphi_2^{(n)}, \phi_1^{(n)}, g_0^{(n)}, g_1^{(n)})$  satisfying
% \begin{IEEEeqnarray}{rCl}
%     \label{eq:covert_constraint}
%    \lim_{n \rightarrow \infty} \delta_{n,w_3} &=& 0, \qquad \forall w_3 \in \mathcal{M}_3 ,\\
%     \lim_{n \rightarrow \infty} P_{ei} & = & 0,\qquad  \forall i\in\{0,1\}.\label{eq:Pei}
% \end{IEEEeqnarray}
% and 
% \begin{IEEEeqnarray}{rCl}
% % \log(M_1}
%  r_1 & \leq &   \liminf_{n \rightarrow \infty} \frac{\log(M_1)}{\sqrt{ n \frac{1}{M_3} \sum_{w_3 = 1}^{M_3} \delta_{n,w_3} }},\\
% % \log(M_2}
%  r_2 & \leq &   \liminf_{n \rightarrow \infty} \frac{\log(M_2)}{\sqrt{ n \frac{1}{M_3} \sum_{w_3 = 1}^{M_3} \delta_{n,w_3} }},\\
% \label{eq:asymp2}
% % \log(M_3}
%  r_3 &\leq& \liminf_{n \rightarrow \infty} \frac{\log(M_3)}{n} ,\\
% % \log(K_1}
% k &\geq&\limsup_{n \rightarrow \infty} \frac{\log(K_1K_2)}{\sqrt{ n \frac{1}{M_3} \sum_{w_3 = 1}^{M_3} \delta_{n,w_3} }}.
% \end{IEEEeqnarray}
% \end{definition}
% Notice that the scaling of the covert rates $r_1$ and $r_2$ are not the usual scaling as is the case for the non-covert rate $r_3$. In particular, covert communication takes place in a zero rate regime, and one cannot send more than $\mathcal{O}(\sqrt{n})$ bits to remain covert, motivating normalisation with $\sqrt{n}$. We further normalize by the average of the covertness constraints as this has a direct impact on the rate.

